A Review on Intelligent Object Perception Methods Combining Knowledge-based Reasoning and Machine Learning

Object perception is a fundamental sub-field of Computer Vision, covering a multitude of individual areas and having contributed high-impact results. While Machine Learning has been traditionally applied to address related problems, recent works also seek ways to integrate knowledge engineering in order to expand the level of intelligence of the visual interpretation of objects, their properties and their relations with their environment. In this paper, we attempt a systematic investigation of how knowledge-based methods contribute to diverse object perception tasks. We review the latest achievements and identify prominent research directions.

==> camera ready latex for arxiv/commonsense.tex <==
%%% CURRENTLY EDITED BY: Theodore

\section{Exploitation of Commonsense Knowledge}

Much of the information presented in a visual scene is not explicitly related with the features captured at the pixel level, but concerns observations implicitly depicted in images. Understanding the structure and dynamics of visual entities requires being able to interpret the semantic and commonsense (CS) features that are relevant, in addition to the low-level information obtained by photorealistic rendering techniques~\cite{vedantam2015learning}. This is a popular conclusion reached within the CV community in the pursue towards achieving visual intelligence. There is a long line of studies that attempt to address the problem of extracting commonsense knowledge from visual scenes or, similarly, of utilizing commonsense inferences to improve scene understanding. In this section, we discuss state-of-the-art approaches that advance the field in these two directions.

\subsection{Mining Commonsense Knowledge from Images}



Even though ML is becoming part of many systems, it is still not able to easily capture CS knowledge from the perceived information. Additional techniques need to be devised to extract this valuable type of knowledge from visual scenes. A combination of textual and visual analysis, which extracts \emph{subject-predicate-object triples (SPO)} about objects recognized in a scene, is addressed in certain studies, e.g., \cite{vedantam2015learning,lin2015don}.  ML classifiers for object recognition are trained on image datasets, while pre-trained NN classifiers help extract SPO triples, by considering both the entities identified by the classifiers and the textual description of the images. 

        
In a different direction, in \cite{sadeghi2015viske} the authors rely on Web images to verify the validity of simple phrases, such as \textit{``horses eat hay''}, analyzing the spatial consistency of the relative configurations of the entities and the relations involved. This unsupervised method is particularly interesting, due to the leverage it offers in automatically enriching CS repositories. In fact, the authors show how CV-based analysis can help improve recall in KBs, such as WordNet, Cyc and ConceptNet, offering a complementary and orthogonal source of evidence.



Aditya et al. (\citeyear{Aditya2018}) %(\citeyear{aditya2015images}) 
 address the problem of generating  linguistic descriptions of images  by utilizing a special type of graph, namely scene description graphs (SDGs). Such graphs are built by  using both low-level information derived using perception methods and high-level features capturing CS knowledge stemming from  the image annotations and  lexical ontological knowledge from Web resources. SDGs produce  object, scene and constituent detection tuples, accompanied by a confidence score; pre-processed background knowledge helps remove noise contained in the detection. A Bayesian Network is utilized, in order for  the dependencies among co-occurring entities and knowledge regarding abstract visual concepts to be captured. Experimental evaluations of the method on the image-sentence alignment quality, i.e., how close the generated description is to the image being described, on Flickr8k, 30k and COCO datasets, showed that the method achieves comparable performance to previous state-of-the-art methods.


\subsection{Commonsense Knowledge in Addressing OP Tasks}

%\textit{Add here SotA papers that show how ML can be empowered by using CS knowledge from text and/or CS repositories.}

State-of-the-art CS-based methodologies improve the performance of a CV system, mainly by taking into account textual descriptions about the entities found in a visual scene or by retrieving semantic information from external sources that is relevant to the image and the task at hand. 

A combination of external Web-based knowledge, text processing and vision analysis is at the core of the study presented in \cite{wang2018fvqa}. The framework annotates objects with a Fast-RNN, trained over the MS COCO dataset. The extracted entities are enriched with (i) knowledge retrieved from Wikipedia, in oder to perform entity classification; (ii) knowledge from WebChild, attempting a comparative analysis between relevant entities; and (iii) CS knowledge obtained from ConceptNet, to create a semantically rich description. The enriched entity is stored in an RDF graph and is used to address a variety of tasks. For instance, the framework has achieved improved accuracy in VQA benchmarks, but also it can be used to generate explanations for its answers. Prominent recent studies, as in~\cite{li2019visual} and \cite{narasimhan2018straight}, also build on the direction of combining textual and visual analysis with the help of knowledge obtained from CS repositories.


Another problem that researchers try to address with the help of CS knowledge is the sparsity of categorical variables in the training datasets. For example, Ramanathan et al. (\citeyear{Ramanathan2015}) utilize a neural network framework that uses different types of cues (linguistic, visual and logical)  in the context of  human actions identification. %Through  the leverage obtained by the detection of the rich semantic relationship between different actions, reasoning about relationships and an extrapolation of unobserved actions from known actions is possible. The generation of  action relationships is further refined  through  the use of a special function  which  combines visual information and logical consistency, resulting in improved performance on diverse action datasets.
Similarly, Lu et al. (\citeyear{Lu2016}) exploit
language priors extracted from the semantic features of an image, in order to facilitate   the  understanding of visual relationships. The proposed model combines  a visual module tailored
to the learning of visual appearance models for  objects and predicates with a language module capable of detecting  semantically  related relationships.% By avoiding the utilization of a very large visual dataset for training, this strategy enabled the method to scale in predicting thousands of types of relationships, outperforming related methodologies on datasets with visual phrases, while also being able to even perform zero-shot learning of visual relations.%. More specifically, the experimental evaluation conducted on visual phrases dataset \cite{} and a newly introduced dataset demonstrated that the method outperformed previous state of the art  methods  and also that it can be used for zero shot learning of visual relationships
 
More recently, Gu et al. (\citeyear{gu2019scene}) utilize  commonsense knowledge stemming from an  external KB in the context of scene graph generation. Namely, a special knowledge-based feature refinement module is used, which incorporates CS knowledge  from ConceptNet for the prediction of object labels consisting of triplets containing the top-K corresponding relationships, the object entity and a weight corresponding to the frequency of the triplet. This strategy, aiming to address the long tail distribution of relationships, differentiates the approach from the linguistic-based ones described previously, managing to showcase improvement in generalizability and accuracy. 
%Furthermore, this approach resulted in an improved generalizability since the object and phrase features that were produced  before the scene generation were more accurate. Specifically, the method was tested on VRD \cite{}  and VG datasets \cite{} and outperformed all  other  state-of-the-art methods.
 
CS knowledge is also used to tackle other CV problems, such as in understanding relevant information about unknown objects existing in a visual scene. In \cite{icarte2017general} or \cite{young2016towards} for instance, external CS Web-based repositories are used as a source for locating relevant information. The general idea in both approaches is to retrieve as much information as possible about the recognizable objects that, based on diverse metrics, are considered semantically close to the unknown ones. $RelatedTo$, $IsA$, $UsedFor$ properties found in ConceptNet, or comment boxes retrieved from DBpedia are all relevant knowledge that can be used for developing semantic similarity measures. Similar to some extent, is the approach presented in \cite{ruiz2016probability}, which relies on RDF graphs with a probabilistic distribution over relations to capture the CS knowledge, but reverts also to a human-supervised learning approach whenever unknown objects are encountered.







==> camera ready latex for arxiv/conclusions.tex <==
%%% CURRENTLY EDITED BY: 





\section{Conclusions}

In this paper, we reviewed approaches that rely on both knowledge-based and data-driven methods, in order to offer solutions to the field of intelligent object perception. By adopting a knowledge-driven, rather than a problem-specific grouping, we analyzed a multitude of approaches that attempt to unify high-level knowledge with diverse machine learning systems. The review revealed open and prominent directions, showing clear evidence that hybrid methods constitute an avenue worth exploring.



%progress in integrating these two fields can indeed be achieved by building on appropriately combined hybrid methodologies. %The example of GNNs is indicative, offering a well-established combination of  model-free and model-based methods, and having achieved prominent results in diverse CV tasks, such as object classification~\cite{Marino2017}, affordance detection~\cite{Chuang2018} and scene understanding~\cite{li2017situation}. Other approaches also present promising behavior, overall supporting the view that hybrid methods constitute an avenue worth exploring.


==> camera ready latex for arxiv/discussion.tex <==
%%% CURRENTLY EDITED BY: 

\section{Open Problems and Research Questions}




\begin{table*}
	\caption{Overview of the reviewed literature}
	\vspace*{0.5cm}
	\label{tbl:overview}
	\centering
	\small
	%\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{|p{5cm}|p{2cm}|p{2.2cm}|p{2cm}|p{1.3cm}|p{2.5cm}| }
		\hline
		\textbf{Indicative Recent Literature} & \textbf{CV Problem Focus}  &  \textbf{ML Methods Applied} & \textbf{KB Methods Applied} & \textbf{KB Contribution} & \textbf{KB-ML Impact}\\
		\hline
		\hline
		

		
		\cite{Chuang2018}, \cite{Ye2017}, \cite{Sawatzky2019}, \cite{Chao2015}, \cite{Ramanathan2015} & affordance detection & CNN, GNN, GGNN  & Knowledge Graphs & 3, 4, 5, 7 & offers new insights\\
		\cite{beetz2018know}, \cite{ramirez2017transferring}, \cite{lemaignan2017artificial}, \cite{agostini2017efficient}, \cite{Moldovan2018} & affordance detection & scoring functions, probabilistic programming models, Bayesian Networks & OWL Ontology & 1, 2, 3, 4, 5, 6, 9 & offers new insights and improves SotA\\
		
		\hline
		\cite{icarte2017general}, \cite{redmon2017yolo9000}, \cite{Liu2018} & object detection & RCNN, CNN & Knowledge Graph, BLN & 1, 3, 4, 5, 8 & offers new insights\\
		\cite{gemignani2016living}, \cite{tenorth2017representations}, \cite{young2016towards}, \cite{beetz2018know}   & object detection & scoring functions, probabilistic programming models & OWL Ontology, DL, MLN & 1, 2, 3, 4, 5, 8, 9 & improves SotA\\
		
		\hline
		\cite{chernova2017situated}, \cite{young2017making}, \cite{Aditya2018} % \cite{aditya2015images}  
		& scene understanding & probabilistic programming, Bayesian Network & BLN & 2, 3, 4, 8 & offers new insights\\
		\cite{gu2019scene}, \cite{li2017situation}, \cite{Chen2018} & scene understanding & GGNN & Knowledge Graph & 3, 4, 7 & improves SotA\\

		
		\hline
		\cite{Krishna2017}, \cite{Zhu2015a}, \cite{li2019visual}, \cite{wu2016ask}, \cite{Wu2018}, \cite{li2017incorporating}, \cite{sadeghi2015viske}, \cite{shah2019kvqa}, \cite{Su2018}, \cite{narasimhan2018straight}, \cite{wang2018fvqa}  & VQA & CNN, LSTM, RCNN & Knowledge Graphs (RDF mostly) & 1, 2, 3, 4, 5, 8 & offers new insights and improves SotA \\
		%\hline
		% \cite{narasimhan2018straight}, \cite{Wang18} & VQA & CNN, LSTM, RCNN & RDF Graph & 2, 3, 4, 5, 6 & offers new insights\\
		 %\hline
		 \cite{vedantam2015learning}, \cite{lin2015don} & VQA & Gausian Mixture Model, SVM &  RDF Graph & 2, 3, 4, 5  & improves SotA\\
		 \cite{Lu2018} & VQA & Gated Recurrent Unit Network &  RDF Graph & 1, 2, 4, 8  & offers new insights\\		 
		 
		 
		\hline
		\cite{Hu2017}, \cite{johnson2017inferring}, \cite{Yi2018}, \cite{Santoro2017} & visual reasoning & Neural Module Network & Symbolic Programming Language & 2, 3, 5 & offers new insights\\
		
		\cite{SuchanMehul17}, \cite{RileySridharan19}, \cite{BasuShakerinGupta20} & visual reasoning, VQA & CNN, RCNN & Non-monotonic logics, ASP & 2, 3, 4, 5, 6, 7, 9 & offers new insights\\
		
		\hline
		\cite{Marino2017}, \cite{Lee2018}, \cite{Wang2018b}  & image classification/ zero-shot recognitions & GGNN, GCN,  & Knowledge Graph, RDF Graph & 1, 2, 5 &  offers new insights and improves SotA\\
		
		\cite{fu2015zero}, \cite{xian2016latent}  & image classification/ zero-shot recognitions & Latent embedding model, Markov Chain Process & Knowledge Graph & 1, 2, 5 &  offers new insights\\
		
		 
		\hline
	\cite{Antanas18}, \cite{antanas2018semantic}, \cite{Moldovan2018}, \cite{Katzouris19}   & affordance learning & scoring functions, probabilistic programming models & FOL, Causal Probabilistic Logic, MLN, Event Calculus & 1, 2, 3, 6, 7, 9 & improves SotA\\
		
		
		\hline\hline

		\multicolumn{6}{l}{\textbf{KB Contribution}: 1:concept abstraction/reuse, 2:complex data querying, 3:spatial reasoning, 4:contextual reasoning,  }\\
		\multicolumn{6}{l}{5:relational reasoning, 6:temporal reasoning, 7:causal reasoning, 8:access to open-domain knowledge, 9:formal semantics}\\
	%\multicolumn{6}{l}{* Only some of the studies}\\
	\end{tabular}
\end{table*}


The review of the state-of-the-art reveals prominent solutions for various OP-related topics, as well as novel contributions that offer new insights (Table~\ref{tbl:overview}). The analysis can also help frame open questions towards combining ML and knowledge-based approaches in the given context. 

\subsection{Obtaining Human Commonsense}


The exploitation of CS knowledge is a characteristic example of a still open research area. Its significance was acknowledged more than two decades ago and the research conducted over the years contributed methods that combine the strengths from diverse fields of AI. At the same time, it is evident that there is still a long way to go; just the coupling of textual and visual embeddings, the mainstream in current VQA related studies, has proven to be a challenging task. Further directions need to also be explored, such as in performing complex forms of CS inferencing or in fusing the huge volume of general knowledge that exists on the Web, while eliminating the bias of information found online.  

Progress in the field of learning from demonstration can prove a vital contribution to CS inferencing and vice versa. Leaving the visual challenges involved aside, this application domain, characterized by the central role of, human mostly, agents, offers theory building opportunities on diverse perspectives. Interaction with human users calls for intuitive means of communication, where high-level, declarative languages seem to offer a natural way of capturing human intuition. Transferring knowledge between high-level languages and low-level models is a key area of investigation for future symbiotic systems and a fruitful domain for combining data-driven and symbolic approaches. 

\subsection{Understanding Causality}

Still, the most demanding outcomes that are expected by the integration of knowledge-based and ML methodologies concern the aspects of causality learning and explainability. Existing works on harvesting causality knowledge do not yet offer convincing models. As argued in~\cite{Pearl18}, ML needs to go beyond the detection of associations, in order to exhibit explainability and counterfactual reasoning. 

The black-box character of ML-based methods hinders the understanding of their behavior, and eventually the acceptance of such systems. For example, recent studies demonstrate the fundamental inability of neural networks to efficiently and robustly learn visual relations, which renders the high performance that networks of this type often achieve worth a closer investigation~\cite{kim2018not,rosenfeld2018elephant}. 
Advancement in exploiting CS knowledge is expected to offer a significant leverage in understanding and reasoning with causal relations. And, of course, transparent reasoning is vital in understanding the abilities and constrains of existing systems. Yet, as indicated in the current review, this latter direction is still not pursued in a coordinated and structured way.




\subsection{Achieving a Tighter Integration}

Ultimately, unifying logical and probabilistic graphical models seems to be at the heart of handling the majority of real-world problems. Recent studies show that even a loosely-coupled integration can achieve better accuracy in classification problems with small datasets in comparison with end-to-end deep networks and comparable accuracy with larger datasets (see e.g., \cite{RileySridharan19,BasuShakerinGupta20}). A tighter integration is highly anticipated, as it will help build systems that learn from data, while still being able to generalize to domains other than the ones trained for. Existing solutions are indeed promising, as for example approaches based on the widely used Markov Logic, which nevertheless introduces limitations on both the theoretical and the practical level \cite{DomingosLowd19}. Its first-order nature, for instance, often contradicts with the non-monotonicity met in CS domains. The support for complex tasks, such as causal, temporal or counterfactual reasoning, in a non-monotonic fashion and over rich conceptual representations unfolds a series of research questions worth exploring in the near future.



%\textit{Our tarapfike home message A:} Progress in KR will offer interoperability, exchange of knowledge and ability for hybrid solutions in MV. Mention the benefits of having representations with formal semantics. Mention the achievements within cognitive robotics projects, such as RoboEarth. Claim that CV in open settings can take advantage of scene understanding involving objects that most probably have been annotated by others, in other settings. Mention also SotA CV papers that are towards this direction

%\textbf{A:} Another, category important category are the systems using Cloud Repositories, which we considered them out of the scope of this symposium therefore are mentioned here. Cloud Repositories could ease the CV module because a system does not need to recognize a new object or understand a human manipulation task, to infer what the system is looking at, as it can use knowledge annotated by others. One of the pioneers in this field was the RoboEarth framework \cite{riazuelo2015roboearth} and OPEN-EASE \cite{beetz2015open}. Even though, scalability issues arise when using knowledge extracted from other platforms, the advantages are many because Cloud Repositories offer semantic information between objects, annotate unknown objects, and overcome problems encountered by spatial or dynamic knowledge \cite{pinacho2018acquiring,bozcuouglu2018exchange,ayari2017contextual}.
  
%\textit{Our take home message B on Commonsense:} Go beyond text+vision? Utilization of Web knowledge? See the Davis ACM paper

%\textbf{A:} CS is a factor which is implemented in a system in order to empower the reasoning and inferencing mechanism, and its flexibility. Recent works show that CS methods based on textual and visual information can reason about the plausibility of an interaction or relation \cite{vedantam2015learning}. Estimate spatial consistency and enrich existing local KB \cite{sadeghi2015viske}. Also, CS methods can make a system hypothesize scenaria to avoid wrong executed tasks \cite{lin2015don}. Utilizing CS and Web Knowledge can assist the reasoning and the perceptual mechanism of the system. It has been shown that Web Knowledge when fused in the system CS methods, it allows to understand unknown objects \cite{icarte2017general,young2016towards}. Find out in what environment the system is \cite{young2017making,chernova2017situated}, and broaden open-domain visual questions \cite{li2017incorporating,wang2018fvqa,li2019visual}. 

%\textit{Our take home message C:} Learning from demonstration is a big field within CV and interacting with users requires high-level, declarative languages that are closer to the human intuition, yet easily translated into low-level representation that can be used as input to CV tools

%\textbf{A:} Learning through human demonstration requires plurality in KR, advanced CV perceiving mechanisms, and ML methods to automatize the procedure after training. Learning sequential tasks as stated in \cite{figueroa2016learning}, requires high-level task demonstration of sequence and low-level parametrization of each action primitive. Then, based on this information more accurate demonstration of the human performed tasks \cite{agostini2017efficient} can be achieved, which can be served as a more representative input for the ML module. Moreover, dynamic growth of ontology KB and flexibility across different demonstration and domain constrains \cite{ramirez2017transferring}.  

%\textit{Our take home message D:} Develop XAI methods that clarify the process of inferencing, a core target in AI. Mention some VQA papers, where scene understanding is based on the semantic analysis of the surrounding objects. But also add papers that improve NNs with explainable features.



%\textit{F:} Far from wanting to downplay the recent successes of DL-based methods, we consider, nonetheless, that their limitations \cite{Marcus2018} render them inappropriate to address, without additional support from other forms of learning, complex problems such as high-level CV tasks. First, their dependency on the training datasets is a major drawback due to the  biases inherent in every dataset \cite{torralba2011unbiased}. Similarly,  the long tail distribution in these datasets is another problem that, although known for long time, has not been resolved.  

%Furthermore,  the black-box character of DL-based methods is another major drawback since it hinders extremely the understanding of their behavior. For example, a recent work demonstrated the fundamental inability of feedforward neural networks to efficiently and robustly learn visual relations, something which renders the high performance that networks of this type achieved in similar taks highly suspicious\cite{kim2018not}. Likewise, the vulnerability in adversarial settings and the easiness with which  they can be manipulated \cite{rosenfeld2018elephant} constitutes  another important shortcoming of these methods.


%In addition, as \cite{Pearl18} argues, since DL  can not go beyond the detection of associations, they are incapable of providing explainability  and counterfactual reasoning. However, both of these features are considered essential for the building of systems capable of exhibiting AGI performance.

==> camera ready latex for arxiv/explainability.tex <==
%%% CURRENTLY EDITED BY: 

\section{Explainability in Reasoning}

\textit{Message: Develop XAI methods that clarify the process of inferencing, a core target in AI}

\textit{Mention some VQA papers, where scene understanding is based on the semantic analysis of the surrounding objects. But also add papers that improve NNs with explainable features}

==> camera ready latex for arxiv/intro.tex <==
%%% CURRENTLY EDITED BY: 

\section{Introduction}

%\textit{ ML and KR: the need to find common grounds is highlighted recently (mention de Giacomo etc). }

%\textit{There are studies that give insights from a rather generic point of view (mention surveys)}

%\textit{Our goal is to focus on MV-related problems (explain why this is important. E.g., make connections with  the targeted objectives of the symposium)}

%\textit{There are MV surveys but do not specifically focus on how KR can help (mention the most important/recent surveys)}

%\textit{Explain our contributions (mention that recent survey we found that is closer to our paper). Explain who are the beneficiaries and why (MV community, KR community, other audiences). Also explain our way of organizing material. We could list here some of the main future directions that will be revealed from our study}

%\textit{Should we mention the AI special issue on robotics?}

Despite the recent sweep of progress in Machine Learning (ML) which is stirring  public imagination about the capabilities of future Artificial Intelligence (AI) systems, the research community seems more composed, in part due to the realization that current achievements are largely based on engineering advancements, and only partly on novel scientific progress. Undoubtedly, the accomplishments are neither small nor temporary; in the latest ``One Hundred Year Study on AI", a panel of renowned AI experts is foreseeing tremendous impact of AI in a multitude of technological and societal domains in the next decades, fueled primarily by systems running ML algorithms~\cite{Stone16AIReport}. Yet, there is still a lot of ground to cover, before we can obtain a deep understanding of how to overcome the limitations of data-driven approaches at a more generic level.

Aiming at exploiting the full potential of AI, a growing body of research is devoted to the idea of integrating ML and knowledge-based approaches. Davies and Marcus (\citeyear{Davis15}) for instance, while discussing the multifaceted challenges related to automating commonsense reasoning, a crucial ability for any intelligent entity operating in real-world conditions, underline the need to combine the strengths of diverse AI approaches from these two fields. Others, as for example Bengio et al. (\citeyear{Bengio19}) and Pearl (\citeyear{Pearl18}), emphasize the inability of Deep Learning to effectively recognize cause and effect relations. Pearl, Geffner (\citeyear{Geffner18}) and recently Lenat\footnote{\url{https://towardsdatascience.com/statistical-learning-and-knowledge-engineering-all-the-way-down-1bb004040114}}, suggest to seek solutions by bridging the gap between model-free, data-intensive learners and knowledge-based models and by building on the synergy between heuristic level and epistemological level languages.%, which will result in more robust and general intelligence systems.

In this paper, we review recent progress in the direction of coupling the strengths of ML and knowledge-based methods, focusing our attention on the topic of Object Perception (OP), an important sub-field of Computer Vision (CV). Tasks related to OP are at the core of a wide spectrum of practical systems and relevant research has traditionally relied on ML to approach the related problems. The recent developments have significantly advanced the field, but, interestingly, state-of-the-art studies try to  integrate symbolic methods, in order to achieve broader visual intelligence. It seems that it is becoming less of a paradox within the CV community that in order to build intelligent vision systems, much of the information needed is not directly observable. %In this respect, the field of CV can be considered an ideal domain to apply what Doug Lenat recently suggested as the way forward; a synergy between heuristic level and epistemological level languages.\footnote{\url{https://towardsdatascience.com/statistical-learning-and-knowledge-engineering-all-the-way-down-1bb004040114}}

Existing surveys on the intersection of ML and knowledge engineering (e.g., \cite{Nickel0TG16}) are indeed very informative, but they usually offer a high-level understanding of the challenges involved. The rich literature on CV reviews, on the other hand, adopts a more problem-specific analysis, studying in detail the requirements of each particular CV task (see e.g., \cite{wu2017visual,herath2017going,liu2018deep}). Only recently was an overview presented that shows how background knowledge can benefit tasks, such as image understanding \cite{Somak19}; our goal is to explore  this direction on the topic of intelligent OP, reporting state-of-the-art achievements and showing how different facets of knowledge-based research can contribute to addressing the rich diversity of OP tasks. 


%Although existing surveys on the intersection of ML and knowledge-engineering are indeed very informative in revealing strengths and weaknesses from a more generic perspective (e.g., \cite{Nickel0TG16}), we believe that by fixing the context on CV tasks and by understanding the particular requirements introduced, we can identify more accurately where the contributions are more effective, and why. This understanding can be transfered to other domains that share similar requirements, as we discuss in Section ??.  

%As a result, this paper is aimed to researchers and engineers from diverse fields wishing to see how far data-driven and knowledge-based systems have reached in addressing a repertoire of practical problems, as well as which directions seem to offer prominent opportunities. The paper is aimed at CV researchers too, as, despite the many and very rich in content surveys in the field (e.g.,\cite{wu2017visual,herath2017going,liu2018deep} ), the majority of reviews adopts a problem-oriented analysis. Only recently an attempt was made to show how studies that utilize background knowledge can assist in image understanding \cite{Somak19}; our goal is to explore in more depth and breadth this direction, touching upon diverse problems in the field of CV. 

\begin{figure}[!h]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{diagram.png}
	\end{center}
	\caption{Organization of thematic areas.}
	\label{fig:diagram}
\end{figure}

The rest of the paper investigates state-of-the-art literature on intelligent OP along the three pillars shown in Figure \ref{fig:diagram}): i) symbolic models, further analyzed from the perspectives of expressive representations, reasoning capacity, and open domain, Web-based knowledge; ii) commonsense knowledge exploitation, a key skill for any intelligent system; and, iii) enhanced learning ability, building on hybrid approaches. By no means should this review be considered exhaustive; inevitably, relevant studies may not have been included. Our intention is to capture a snapshot of the most recent research trends, discussing studies that improve previous results or offer new insights, hoping to provide a starting point for following the interesting progress currently underway, while giving pointers to directions that seem worth investigating. In this respect, the paper concludes with a discussion on open questions and prominent research directions. Table~\ref{tbl:overview} at the end summarizes the reviewed literature.

==> camera ready latex for arxiv/learning.tex <==
%%% CURRENTLY EDITED BY: 

\section{Ability to Learn New Knowledge}

The majority of state-of-the-art studies covered in the previous sections exploit a loosely-coupled combination of ML and knowledge-based methodologies. A tighter integration of methodologies of the two fields is expected to achieve much broader impact, especially in the process of learning. In the sequel, we consider  prominent attempts towards this direction, originating  either from a model-free standpoint or from a more declarative, inductive-based perspective.

\subsection{Model-Free Learning} 




 


%\textit{Message:} Should be something related to improving scalability issues, avoiding having to train many classifies etc

Recent studies devise methods that attempt to exploit information contained in higher-level representations, in order to improve scalability and generalization for tasks, such as Zero-Shot Learning (ZSL). ZSL is the problem of recognizing objects for which no visual examples have been obtained and is typically achieved by exploring a semantic embedding space, e.g., attribute or semantic word vector space.

% where the training of discrete classifiers is con

For example, Fu et al. (\citeyear{fu2015zero})  utilize a semantic class label graph, which results in a more accurate distance metric in the semantic embedding space and an improved performance in ZSL. 
%\cite{huang2015learning} Should we refer to this work
Likewise, Xian et al. (\citeyear{xian2016latent}) address the same problem by proposing a novel latent embedding model, which  learns a compatibility function between the image and semantic (class) embeddings. The model utilizes image and class-level side-information that is either collected through human annotation or through an unsupervised way from a Web repository of text corpora. 



Lee et al. (\citeyear{Lee2018}) propose a novel deep learning architecture for multi-label ZSL, which relies on KGs for the discovery of the  relationships between multiple classes of objects.  The KG is built on knowledge stemming from   WordNet  and contains
3 types of label relations, super-subordinate, positive correlation, and negative correlation. The KG is coupled to a GGNN-type module for predicting labels. %Similarly to other GGNNs, the structure of the KG along with the incorporated information  contributes to the updating of the GGNN  module nodes during its training.  %The experimental testing of the  model reported  improved performance on the  task of multi-label classification and performance comparable state-of-the-art approaches on  challenging problem of ML-ZSL.


In the same vein, Wang, Ye and Gupta (\citeyear{Wang2018b}) exploit the information contained in KGs about unseen objects, in order to infer visual attributes that enable their detection.  The KG nodes correspond  to  semantic categories and the edges to semantic relationships, whereas the input to each node is the vector representation (semantic embedding)
of each category. A GCN is used to transfer information  between different categories. %with an approach similar to that described for GGNN previously.
This way, by utilizing the   semantic embeddings of a novel category, the method can link categories in the KG to familiar ones  and, thus, infer its attributes. The experimental evaluation demonstrated a significant improvement on the ImageNet dataset, while the ablation studies indicated that  the incorporation of KGs enabled the system to learn meaningful classifiers on top of semantic embeddings.

In \cite{Marino2017},  the use of structured prior knowledge led to  improved performance on the task of  multi-label image classification.  The KG is built using WordNet for the concepts and Visual Genome for the relations among them. An interesting aspect of this study is the introduction of a novel NN architecture, Graph Search Neural Network, as a means to efficiently incorporate large knowledge graphs, in order to be exploited for CV tasks. 

\subsection{Inductive Learning}
The benefits of developing intelligent visual components with reasoning and learning abilities are becoming evident in broader to CV domains, such as in the field of Robotics. This conclusion was nicely demonstrated in a recent special issue of the AI Journal~\cite{AIRoboticsSP17}, where causality-based reasoning emerged as a key contribution. It is, therefore, interesting to investigate how the recent trend in combining knowledge-based representations with model-free models for the development of intelligent robots is making an impact in related OP research. 
 
 
%The benefits of developing intelligent components with reasoning abilities start to become widely acceptable in the CV community, as the previous subsection showed. Even more evident such benefits are in broader domains, where CV plays a key role; the field of Robotics is probably the most characteristic example, as was nicely demonstrated in a recent special issue of the AI Journal \cite{AIRoboticsSP17}. Since Robotics traditionally progressed in close collaboration with CV, it is interesting to investigate how the recent trend in combining knowledge-based representations with model-free models for the development of intelligent robots with cognitive skills is making an impact in related CV research.

A highly prominent line of research for modeling uncertainty and high-level action knowledge is focusing on combining expressive logical probabilistic formalisms, ontological models and ML. In~\cite{Antanas18} for example, the system learns probabilistic first-order rules describing relational affordances and pre-grasp configurations from uncertain video data. It uses the ProbFOIL+ rule learner, along with a simple ontology capturing object categories. 

More recently, Moldovan et al. (\citeyear{Moldovan2018}) significantly extended this approach, using the Distributional Clauses (DCs) formalism that integrates logic programming and probability theory. DCs can use both continuous and discrete variables, which is highly appropriate for modeling uncertainty, in comparison for instance to ProbLog, which is commonly found in relevant literature. Compared to approaches that model affordances with Bayesian Networks, this approach scales much better, but most importantly, due to its relational nature, structural parts of the theory, such as the abstract action-effect rules, can be transferred to similar domains without the need to be learned again.

A similar objective is pursued by Katzouris et al. (\citeyear{Katzouris19}), who propose an abductive-inductive incremental algorithm for learning and revising causal rules, in the form of Event Calculus programs. The Event Calculus is a highly expressive, non-monotonic formalism for capturing causal and temporal relations in dynamic domains. The approach uses the XHAIL system as a basis, but sacrifices completeness due to its incremental nature. Yet, it is able to learn weighted causal temporal rules, in the form of Markov Logic Networks, scaling up to large volumes of sequential data with a time-like structure.

Also worth mentioning is the study of Antanas et al. (\citeyear{antanas2018semantic}), which instead of learning how to map visual perceptions to task-dependent grasps, it uses a probabilistic logic module to semantically reason about the most likely object part to be grasped, given the object properties and task constraints. The approach models rules in Causal Probabilistic logic, implemented in ProbLog, in order to reason about object categories, about the most affordable tasks and about the best semantic pre-grasps. %Similar to DCs mentioned before, this logic is more compact, models complex uncertain dependencies and is more intuitive, due to its declarative nature, in comparison to graphical models, such as Markov or Bayesian Networks.


==> camera ready latex for arxiv/representation.tex <==
%%% CURRENTLY EDITED BY: 

\section{Exploitation of Symbolic Models}

%\textit{Message A:} Richer representations help achieve better results (we will define what richer means, e.g., different types of graph edges, such as properties and inheritance, formal semantics etc). How? E.g., a) by abstracting concepts related to context awareness, spatial relations, motion, human behavior etc. we alleviate performance/scalability issues whenever too much detail is not needed, b) by supporting different types of reasoning, such as prediction or diagnosis building on causal relations, c) by making more complex queries etc. Describe also categories of CV problems addressed, types of representations that have been used

The scope of OP research ranges over a wide spectrum of problems, from object, action and affordance detection, to localization and recognition in images, to motion and structure inference in videos, to scene understanding and visual reasoning. Traditionally, OP relied on ML methodologies to find patterns in realms of data, taking as input feature vectors representing entities in terms of numeric or categorical (membership to a more general class) attributes. 

In this section, we discuss how high-level knowledge related to visual entities can improve the performance of OP algorithms in manifold ways. We start by reviewing  state-of-the-art in coupling data-driven approaches and rich knowledge representations about aspects such as context, space and affordances. %We, then consider the level of complex querying and reasoning that has been achieved on top of such representations. Finally, we explore how more generic Web-based knowledge sources are employed in an attempt to address similar problems.

\subsection{Expressive Representations of Knowledge}
Although the notion of a representation is rather general, the modeling of relational knowledge in the form of individuals (entities) and their associated relations is well-studied in AI, especially in the context of symbolic representations (see for instance \cite{vanHarmelenLifHandbook07,Brachman04book}). The goal is to offer the level of abstraction needed to design a system versatile enough to adapt to the requirements of a particular domain, yet rigid enough to be encoded in a computer program, having clear semantics and elegant properties \cite{Dean95book}. As a result, \textit{expressiveness}, i.e., what can or cannot be represented in a given model, and \textit{computation}, i.e., how fast conclusions are drawn or which statements can be evaluated by algorithms guaranteed to terminate, are two, often competing, aspects to be taken into consideration. 

The form of the representational model applied plays a decisive role on such considerations, affecting the richness of semantics that can be captured. While the range of models varies significantly, even relatively shallow representations have proven to offer improvements in the performance of OP methodologies (see for example \cite{deng2014large,Feifei14,zhu2015building,redmon2017yolo9000}). Models as simple as  relational tables or flat weighted graphs, but also more complex multi-relational graphs, often called Knowledge Graphs (KGs), or even semantically-rich conceptualizations with formal semantics, often called ontologies, are proposed in the relevant literature. In the sequel, we refer to any model that offers at least a basic structuring of data as a Knowledge Base (KB).





%While the range of representation models varies significantly, even relatively shallow representations have proven to offer improvements in the performance of CV methodologies, as Zhu, Fathi and Fei-Fei (\citeyear{Feifei14}) first showed in a principled way. The authors trained a custom small-scale graph-based representation, based on Markov Logic Networks, in order to capture physical, visual and categorical attributes of objects. Using this model as KB, they presented concrete evidence that tasks, such as zero-shot affordance prediction or object recognition, can be successfully achieved without having to train separate classifiers for each task or new label. The approach was interesting also because it offered a casting of Markov Random Fields (MRFs), a popular model within the CV community for representing joint distributions among multimodal variables, into a first-order representation that can be used for statistical relational learning. Despite the lack of formal semantics for querying the underlying data, which restricted the generality of the methodology, the approach was latter shown to scale well to half billion variables and millions of parameters \cite{zhu2015building}. 

%Another early study that showcased the significance of high-level representations was based on a new graph-based formalism, namely Hierarchy and Exclusion graphs \cite{deng2014large}, which could model subsumption relations, mutual exclusion and overlapping entities. This model was capable of exploiting the semantic knowledge that was extracted by the labeling of objects within an image, in order to perform inference and prediction, resulting to state-of-the art performance in image classification tasks  and inspiring a host of future works, e.g., \cite{Wang2018b,fu2015zero,ramanathan2015learning}. 

%Finally, a method that caused a paradigm shift in relevant literature is given in \cite{redmon2017yolo9000}, where the utilization of a very simple and straightforward higher-level representation yielded significant improvement in the task of object detection. In this case, the representation was inspired by the  WordNet concept graph and consisted of a hierarchical word tree of visual concepts.

%was \cite{deng2014large} where a new formalism, Hierarchy and Exclusion graphs, was introduced which was capable of exploiting the semantic knowledge that can be extracted by the labeling of objects within an image. This novel approach  led to state-of-the art performance in image classification tasks  inspiring a host of   works \cite{Wang2018b,fu2015zero,ramanathan2015learning}. %reformulation of soa bechause it was 2014?



\subsubsection{Utilization of Contextual Knowledge} Context awareness is the ability of a system to understand the state of the environment, and to perceive the interplay of the entities inhabiting it. This feature offers advantages in accomplishing inference tasks, but also enhances a system in
terms of reusability, as contextual knowledge enables it to adapt to new situations and environments that resemble known ones.

A preliminary approach towards this direction utilized a special semantic fusion network, which combined novel object- and scene-based information and was able to capture relationships between video class labels and semantic entities (objects and scenes) \cite{Wu_2016_CVPR}. This was a Convolutional Neural Network (CNN) consisting of three layers, with the first layer detecting low-level features, the second layer object features and the third layer scene features. Although no symbolic representation was applied, this modeling of abstraction layers for the representation of the information depicted in an image is similar to the hierarchical structuring of knowledge used by  top-down methods.

In a similar style, Liu et al. (\citeyear{Liu2018}) recently attempted to address the problem of object detection by proposing an algorithm that exploits jointly the context of a visual scene and an object's relationships. Such features are typically taken into consideration in isolation by most object detection methods. The algorithm uses a CNN-based framework tailored for object detection and combines it with a graphical model designed for the inference of object states. A special graph is created for each image in the training set, with  nodes corresponding to objects and  edges to object relationships. The intuition behind this approach is that the graph's topology enables an object state to be determined not only by its low-level characteristics (appearance details),  but also  by the states of other objects interacting with it and by the overall scene context. %In this novel structure network produced from the coupling of the graph module  with R-CNN, the information referring  either to scene context 	or to  objects  states and relationships can  be propagated in a iterative manner and, thus, can  enhance the object task detection. 
The experimental evaluation conducted on different datasets underscored the importance of knowledge stemming from local and global context. 

%Currently, a collection of prominent state-of-the-art approaches are oriented towards Gated Graph Neural Networks (GGNNs) , in order to integrate contextual knowledge in the training of a system. GGNNs are a special type of NNs tailored to the learning of information  encoded  in a graph. Each node of a GGNN corresponds to a hidden state vector that is updated in a iterative way. At each time step of the training procedure, the history of the node, along with any incoming message from nodes with which it is linked, determines the way that the hidden state of a node will be updated. These updates are applied simultaneously to all nodes in the graph at each propagation step.  After the number of prescribed propagation steps have been concluded, the output of the network is produced as a function of  its nodes hidden states. This procedure differentiates CNNs from standard Recurrent Neural Network, since in the latter the information moves only in one direction and only one node is updated per time step.

Currently, a collection of prominent approaches
are oriented towards Gated Graph Neural Networks
(GGNNs) \cite{li2015gated}, a variation of Gated Neural
Networks (GNNs) \cite{scarselli2008graph}, in order to integrate contextual knowledge in the training of a system. GNNs are a special type of NNs tailored to the learning of information
encoded in a graph. In GGNNs, each node corresponds
to a hidden state vector that is updated in a iterative way. % At each time step of the training process, the history of the node, along with any incoming message from nodes with which it is linked, determines the way that the hidden state of a node will be updated. These updates are applied simultaneously to all nodes in the graph at each propagation step. After the number of prescribed propagation steps concludes, the output of the network is produced as a function of its nodes hidden states. The building block of GGNNs are gated recurrent units which serve as recurrent functions, with recurrence being applied for a fixed number of steps. Therefore, there is no need for constraining the parameters in order to ensure convergence. 
Two features that differentiate GGNNs from standard Recurrent Neural Networks (RNNs), which also use the mechanism of recurrence, is that in the former information can move bi-directionally and that many nodes can be updated per step.

Chuang et al. (\citeyear{Chuang2018}) propose a GGNN-based method which exploits  contextual information, such as the types of objects and their spatial relations, in order to detect action-object affordances. In the same vein, Ye et al. (\citeyear{Ye2017}) utilize a two-stage pipeline built around a CNN to detect functional areas in indoor scenes. More recently, Sawatzky et al. (\citeyear{Sawatzky2019}) utilized a  GGNN, % to exploit the appearance of each object as well as the global context of all present objects in the scene.
which takes into account the global context of a scene and infers the affordances of the contained objects. It also proposes the most suitable object for a specific task. The authors prove that this approach yields better results compared to methods that rely solely  on the results of an object classification algorithm.

In \cite{li2017situation}, an approach aiming to perform situation recognition is presented, based on the detection of human-object interactions. The goal is to predict the most representative verb to describe what is taking place in a scene, capturing also relevant semantic information (roles), such as the actor, the source and target of the action, etc. The authors utilize a GGNN, which enables combined reasoning about verbs and their roles through the iterative propagation of messages along the edges. 

\subsubsection{Spatial Contextual Knowledge} A particular type of contextual knowledge concerns the spatial properties of the entities populating a visual scene. These may involve simple spatial relations, such as ``object $x$ is usually part of object $y$'' and ``object $x$ is usually situated near the objects $x_1,\dots,x_n$'', but also semantically enriched statements, such as ``objects of type $x$ are usually found inside object $z$ (e.g., in the fridge), located in room $y$''. Due to the ubiquitous nature of spatial data in practical domains, such relations are often captured as a separate class of context.

%Due to the ubiquitous nature of spatial data in practical domains, such relations are often captured also as a separate class of context. Spatial information, is the information related to the object position in the environment. For instance , or between objects:  for $n \in \mathbb{N}$, or the class of an object: \emph{the object x is-a instance of class X}. This kind of information when fused in a probabilistic knowledge base gives great flexibility to a system. 

Semantic spatial knowledge, when fused with low-level metric information, gives great flexibility to a system. This is demonstrated in the study of Gemignani et al. (\citeyear{gemignani2016living}), where a novel representation is introduced that combines the metric information of the environment with the symbolic data that conveys meaning to the entities inhabiting it, as well as with topological graphs. Although delivering a generic model with clear semantics is not their main objective, the resulting integrated representation enables a system to perform high-level spatial reasoning, as well as to understand target locations and positions of objects in the environment.

Generality is the aim of the model proposed by Tenorth and Beetz (\citeyear{tenorth2017representations}), which uses an OWL ontology, combining information from  OpenCyc and other Web sources that help compile new classes while forming the environmental map. The main reasoning mechanisms of this study is Prolog, although probabilistic reasoners are also used to tackle fuzzy information or uncertain relations. %, such as \emph{“A living room is a room with exactly one sofa and at least one TV”}, what happens if the living room does not have a TV? how will the system then classify the room. 
A CV system annotates objects based on their shape, their distances and the dimension of the environment, 
%%%AAA: What is meant by "dimension of the environment"?
using a monotonic Description Logic (DL), to build the environmental map. %The system then learns how to manipulate the objects in the environment. 
As a result, a coherent and well-formalized representation of environments is achieved, which can offer high-quality datasets for training data-driven models. The use of DL can also offer a wide spectrum of spatial reasoning capabilities with well-specified properties and formal semantics.
%Also, the high level interaction and reasoning that the system offers to the user which can be supported by grounded facts as learning evolves. Furthermore, these systems are capable of representing and reason more realistically about objects spatial and qualitative representations (i.e. where an object is comparing with others "next to, below, behind, etc."), object geometry and manipulation area. \TP{I need to rephrase this section, to make the messages clearer.}

Adopting a different approach, the KG given in~\cite{Chen2018} enables spatial reasoning both in a local and a global context which, in turn, results in improved performance in semantic scene understanding. The proposed framework consists of two  distinct modules, one  focusing on local regions of the image and one dealing with the whole image. The local module is convolution-based, analyzing small regions in the image, whereas the basic component of the global module is a KG representing regions and classes as nodes, capturing spatial and semantic relations. % (the authors experimented with two versions, one based    on ADE  and one on Visual Genome Dataset (VG) respectively) which, in turn,  enabled the encoding of spatial and semantic relationships.    
According to the experimental evaluation performed on the ADE and Visual Genome datasets, the network achieves better performance over other CNN-based baselines for region classification, by a margin which sometimes is  close to 10\%. According to the ablation study, the most decisive factor for the framework's performance was the KG.

\subsubsection{Modeling Affordances} %\TP{Maybe mention some surveys here}
Building on the geometrical structure and physical properties of objects, such as rigidity and hollowness, the representation of affordances helps develop systems that can reason about how human-level tasks are performed. While ML is invaluable for automating the process of learning from example when  data is available, rich representations can generalize and reuse the obtained models in situations where data-based training is not possible. 

One of the first studies that demonstrated that even very basic semantic models can improve  the performance of recognizing  human-object interaction was~\cite{Chao2015}. The authors succeeded in boosting the performance of visual classifiers by exploiting the compositionality and concurrency of semantic concepts contained in images. 

KNOWROB 2.0~\cite{beetz2018know}, which is the result of a series of research activities in the field of Cognitive Robotics, is an excellent example of integrating top-down knowledge engineering with bottom-up information structuring, involving, among others, a variety of CV tasks. A combination of KBs of different granularity helps the KNOWROB 2.0 framework capture rich models of the world. %The framework combines an inner world KB with objects 6D poses, equipped with a physics engine; a virtual KB for the state of the environment; a logic KB, which contains abstracted symbolic sensor and action data with logical axioms and an inference mechanism; and an episodic memory KB with past collected experiences  that empowers the system's visual and cognitive skills. 
 The representation of high-level knowledge is based on OWL-DL ontologies, a decidable fragment of First-order Logic (FOL), yet adequately expressive for most practical domains. The KBs enable the system to answer questions, such as \emph{``how to pick up the cup'', ``Which body part to use''} etc. The authors provide evidence that learning human manipulation tasks on existing methods can be boosted by using symbolic level structured knowledge. %, so that the system can formalize learning problems and generate training datasets based on their episodic memories. %An interface for coupling the model with a multitude of ML algorithms (through the Weka software) is also provided. % Also, KNOWROB 2.0 offers an interface to the ML framework Weka. Comparing to other systems, this framework acquires open-ended manipulation skill and commonsense knowledge as they managed to fuse realistic representation of objects, together with self location information, timesteps for the actions, and episodic memories. Additionally, the new method of learning thought episodic memories is presented for the first time.

%A new way of detecting and learning relational affordances is presented in recent studies (e.g., \cite{moldovan2018relational,daruna2019robocse}). The idea is to use a local KB \TP{what is stored in the local KB} and an external KB, such as AI2THOR, %cite if remains which contains real-world environments, from where knowledge about affordances and locations of objects can be mined \TP{how? by querying? by training a dedicated classifier?}. The knowledge is then stored in Bayesian Logic Networks \TP{is this the local KB?} that interacts with discrete and continuous variables (otherwise called Linear Continuous Gaussian Bayesian Networks) \TP{what do you mean that the knowledge interacts with variables?}. The biggest contribution of this line of research is that general ML and data-driven methods can be trained to understand semantics between human motion and objects \TP{this seems really interesting. can you explain a bit more?}, avoiding having to train separate classifiers. %A factor that will help avoid training a classifier for human motion, then another one for object properties, and maybe a third one that finds correlations between the two previous ones. \TP{I need to read this again to understand it.}

A recently proposed novel representation model that manages to balance between concept abstraction, uncertainty modeling and scalability is given in~\cite{daruna2019robocse}. The so called RoboCSE framework encodes the abstract, semantic knowledge of an environment, i.e., the main concepts and their relations, such as location, material and affordance, obtained by observations, simulations, or even from external sources, into \textit{multi-relational embeddings}. These embeddings are used to represent the knowledge graph of the domain in vector space, encoding vertices that represent entities as vectors and edges that represent relations as mappings. While the majority of similar approaches rely on Bayesian Logic Networks and Markov Logic Networks, suffering from well-known intractability problems, the authors prove that their model is highly scalable, robust to uncertainty, and generalizes learned semantics. 

%\cite{Koppula2016}  harnessed object affordances in the context of human action anticipation,  by incorporating them in an   conditional random field (CRF) which was used for the prediction of the outcomes of activities. More in detail, the affordances were utilized   w.r.t.   relative position of  objects  and their temporal motions trajectories during  activities.


%\subsubsection{Modeling Grasping Areas}

%Other studies employ a causal probabilistic logic %a citation maybe here to infer grasping areas and object functionalities, which is often formalized with the help of ProbLog as a symbolic language and Bayesian Networks for representing relations. The existence of a probabilistic KB enables a knowledge-based system to make inferences and perform learning, having full support to the uncertainty returned by a CV module. Learning in these cases is performed with low-level learning visual based features by annotating ground facts about the objects shape and geometry \cite{antanas2018semantic}, or a combination of NN trained for grasping region classification and noise removal on the object shape \cite{gupta2018robot}. \TP{I don't understand this sentence. Please be more specific how learning is performed} The combination of high-level reasoning and low-level learning for system grasping has led to significant improvement on grasping tasks, e.g., by a 33\% over baseline models, such as DexNet.

%even when incomplete information has been returned by CV, support generalization, reduce the training data, and be memory efficient. Learning in these cases is performed with low-level learning visual based features by annotating ground facts about the objects shape and geometry \cite{antanas2018semantic}, or a combination of NN trained for grasping region classification and noise removal on the object shape \cite{gupta2018robot}. Where they use Bayesian Networks as KR that learn to annotate grasping region. The innovation here is the new probabilistic approach that combines high-level reasoning and low-level learning for system grasping, and the 33\% improvement over baseline models such as DexNet.% Cite may be needed here.




%\subsubsection{Combining Knowledge in Human Demonstration Use Cases} 

Learning from demonstration, or imitation learning, is a relevant, yet broader objective, which introduces interesting opportunities and challenges to a CV system (see \cite{Torabi19,ravichandar2019lfd}). Purely ML-based methods constitute the predominant research direction, and only few state-of-the-art studies utilize knowledge-based methods, taking advantage of the reusability and generalization of the learned information. A popular choice is to deploy expressive OWL-DL \cite{ramirez2017transferring,lemaignan2017artificial} or pure DL \cite{agostini2017efficient} representations to capture world knowledge. The CV modules are assigned the task to extract information about the state of the environment, the expert agent's pose and location, grasping areas of objects, affordances, shapes etc. On top of these, the coupling with knowledge-based systems assists in visual interpretation, for example to track human motion, to semantically annotate  the movement (i.e., ``how the human performs the action'') or to understand if a task is doable in a given setting. These studies show that such representations enable a system to reuse the learned knowledge in diverse settings and under different conditions, without having to re-train classifiers from scratch. Moreover, complex queries can be answered, a topic discussed in the next subsection.

%Many studies to generalize the knowledge learned from human demonstration, where developed using OWL ontologies with DL \cite{ramirez2017transferring}, more specifically \cite{lemaignan2017artificial} uses OpenRobot Commonsense Ontology%cite maybe here
%an ontology that contains information that allows a robotic platform to perform human scaled tasks, or just DL representation \cite{agostini2017efficient}. CV in these cases tracks human motion, annotates the semantic information in the movement (i.e. "how the human performs the action"), as well as self-location in order for the system to understand if a task is doable from its current position. The purpose of these systems is to extract information related to the state of the environment, human pose and location, grasping area of the object, affordances, shapes, and dimensions. Learning takes place after the information is perceived by the system, the advantages is that the system is learning in real-time, therefore the human can control the learning procedure and training data. Moreover, the system can re-evaluate what it has learned if it is annotated as wrong. These systems can infer the semantics of an action regardless the demonstrator, this means that the same human-scaled action can be performed by a man or a woman and the system would infer it as the same action. Moreover, they achieve multi-modal and interactive symbol grounding where the system observes, builds and maintains knowledge about its human partners perspectives and affordances, and it can in real-time answer user queries related with the progress of the action. For instance the user is carrying some boxes and asks the system where empty space in the room exists that will fit the boxes. This is achieved by grounding the knowledge perceived by their speech recognition (Google API speech recognition), affordances computation with predefined templates existing in their KB, and logic inferences provided by the information inside their ontology.

%\TP{I decided to omit it, it is just a short paper. I searched a bit their publications and did not find anything newer. I found some interesting surveys on Learning from demonstration, though :) }
%Additionally, automatic task segmentation and action primitive discovery, by learning a probabilistic representation of action sequence is presented in \cite{figueroa2016learning}. Where they use a Bayesian Non-Parametric approach for KR, this allows the system to work and learn from demonstration over incomplete and uncertain information, and allow learning be independent of a priori knowledge of model parameters such as the number of hidden states. Their algorithm outputs a set of unique action primitives and their corresponding segmented data, as well as their transition probabilities which are used for learning. Action primitives are consider the atomic actions performed at each time step (e.g. grab, lift, etc). The result is a framework, which can learn complex sequential tasks with a probabilistic logic, such as preparing a pizza, from human demonstration with less demonstrations comparing to other frameworks. \TP{I would omit this. It seems isolated from the previous studies, and is not clear why it is important. If you object, please make improvements}


  

\subsection{Reasoning over Expressive KBs}
Encoding knowledge in a semantically structured way is only part of the story; 
%Apart from encoding knowledge in a semantically structured way, thus enabling data reuse and avoiding having to train separate classifiers for each type of visual entity, as discussed before, 
a rich representation model can also offer inference capabilities to a CV system, which are needed for accomplishing complex tasks, such as scene understanding, or simpler tasks under realistic conditions, such as scene analysis with occlusions, noisy or erroneous input etc. A reasoning system can be used to connect the dots that relate concepts together when only partial observation is available, especially in data-scarce situations, where annotated data are not sufficiently many. In such situations, the compositionality of information, an inherent characteristic of the entities encountered in visual domains, can be exploited by applying reasoning mechanisms.% Purely ontological inference is not always capable for capturing the complexity and uncertainty of visual domains; state-of-the-art approaches are coupling data-driven models with symbolic inferencing in a multitude of ways.

\subsubsection{Complex Query Answering}
%\TP{The intro is very good in this subsection. But then I miss the valuable messages that we give to our reader from our review. I somehow was expecting to see methods that try to analyze text for instance, that use WordNet or DBPedia to enrich the analysis with the meaning of concepts etc.. Also, I recall from the few papers that I read about VQA that LSTM NNs were among the most popular ML methods used and I thought that a clustering of studies would be present here. Instead, what we have is ``approach X did this. Approach Y did that'', without a clear connection among them. I am not sure what the message is that we expect the reader will find valuable. Please try to come up with what VQA methods have in common and let's discuss how we can work this subsection out. Find for instance categories of questions that can be answered effectively and categories that are more difficult to address.}
Probably the field that highlights more clearly the needs and challenges faced by a CV system in answering complex queries about a visual scene is the field of Visual Question Answering (VQA). VQA was recently introduced as a collection of benchmark image-based open-domain questions that, in order to be answered, call for a deep understanding of the visual setting. VQA goes beyond traditional CV, since apart from   image analysis, the proposed methods apply also a repertoire of AI techniques, such as Natural Language Processing, in order to correctly analyze the textual form of the question, and inferencing, in order to interpret the purpose and intentions of the entities acting in the scene~\cite{Krishna2017}. The challenges posed by this field are complex and multifaceted, a fact which is also demonstrated by the rather poor performance of state-of-the-art-systems in comparison to humans. VQA is probably the area of CV that has drawn the most inspiration from symbolic AI approaches to date. % Specifically, Symbolic-AI ideas, such as KG, semantic knowledge and ,have been utilized both in the creation of datasets and benchmarks and, also, in the devising of VQA systems.  Some  examples of this approach that we considered indicative are the following.


An indicative example is the approach recently presented by Wu et al. (\citeyear{Wu2018}), who introduced a VQA model combining observations obtained from the image with information extracted from a general KB, namely DBpedia. Given an image-question
pair, a CNN is utilized to predict a set of attributes from the image, i.e., the most recognizable objects in the image, in terms of clarity and size. Consequently,  a series of captions based on the attributes is generated, which is then used to extract relevant information from DBpedia through appropriately formulated queries. In a similar style, in \cite{narasimhan2018straight} an external RDF repository is used to retrieve properties of visual concepts, such as category, used for, created by, etc. The technique utilizes a Graph Convolution Network
(GCN), a variation of GNN, before producing an answer. In both cases, the ablation analysis reveals the impact of the KB in improving performance.



Other types of questions in VQA require inferencing about the properties of the objects depicted in an image. For example, queries such as \emph{``How is the man going to work?"} or more complex queries, such as \emph{``When did the plane land?"}, have been the subject of the study presented by Krishna et al. (\citeyear{Krishna2017}), who introduced the Visual Genome dataset and a VQA method. In fact, this is one of the first studies to bring a model trained on an RDF-based scene graph that had good recall results to all \emph{What, Where, When, Who, Why, How} queries. Even further, Su et al. (\citeyear{Su2018}) introduced the visual knowledge memory
network (VKMN) in order to handle questions, whose answers
 cannot be directly inferred from the image
visual content but require reasoning over structured human knowledge. 

%Some studies show us some important methods on how to answer VQA. Visual Genome \cite{krishna2017visual} and Visual7W \cite{zhu2016visual7w} are two of those. The former is a dataset in which objects, attributes, and properties between objects are annotated. The dataset is a combination of MS COCO%Cite  and YFCC100M%Cite, and allows for a multi-perspective study of an image, from pixel-level information to even deeper cognitive tasks like question answering. The answer for a query is returned using a correlation of: (1) region, how much space an object occupies, (2) objects, what objects are in the image, (3) attribute, some characteristic are more common between some objects, (4) properties, some properties are more common between objects, statistics which can eliminate some candidate answers, and an SVM that finds similarity between the Q and the A vector representations. 

%They use scene graphs as their KR which can also be consider a dense representation of knowledge for the image. General ML methods for QA can be benefited to answer more complex queries about objects and object properties inside an image, if they are trained over the knowledge contained in the scene graph of the dataset. Their study managed to tackle VQA problems that require inferencing relation between objects in the picture, such as \emph{"How is the man going to work?"} or even more complex queries such as \emph{"When did the plane landed?"}. More specifically, they were one of the first studies to bring a model trained on their scene graph knowledge that had good recall results to all \emph{What, Where, When, Who, Why, How} queries, and also present a dataset with images containing the information needed to train a ML model.  

%While the latter, is based on the former, being a combination of MS COCO, and Visual Genome. Unfortunately they do not state their KR method. A CNN is trained to recognize the bounding boxes of the objects in the images. Then, information returned by the CNN together with the query vector representation are given to an LSTM network to derive the final answer. Learning holds the same benefits as before. An important and innovative aspect of this framework is the attention-based model for grounding the QA, where the visual QA is grounded as a region in the image. This helps extract more specific relations of objects and broaden the inferencing mechanism, and thus as shown in their experiments achieve even better results at finding the correct A for the Q. They achieve an overall 0.556\% over all question categories a difference of 0.115\% with the previous ones. Also, it should be noticed that both rely on Amazon Mechanical Turk to create the QA pairs and the labelling of attributes, objects, and objects regions in the image.



The importance of capturing the semantic knowledge in VQA collections led also to the creation of the Relation-VQA dataset \cite{Lu2018}, which extends Visual Genome with a special module measuring the semantic similarity of images. In contrast to methods mining  only  concepts or attributes, this model extracts  relation facts related to both concepts and attributes. The experimental evaluation conducted on VQA and COCO dataset showed that the method outperformed other state-of-the-art ones. Moreover, the ablation studies show that the incorporated semantic knowledge was crucial for the performance of the network.










Despite its increasing popularity, the VQA field is still hard to confront. The generality of existing methods is also questioned~\cite{Goyal2019}. %For example, in \cite{Goyal2019}) a serious concern is raised whether the training of existing systems is biased, due to the unbalanced content of existing datasets, which favors a very small number of categories that constitute the correct answer for the majority of the questions, offering hints to the training processes. 
Developing generic solutions, less tightly coupled to specific datasets, will definitely benefit the pursuit towards broader visual intelligence.  

 \subsubsection{Visual Reasoning} A task related to  VQA  that has gained popularity in recent  years is that of Visual  Reasoning %\footnote{Instead of the term VR, in some works the term VQA is used. However, we consider that these works belong to VR, since they are tested in standard VR benchmarks such as \cite{Johnson2016}.} 
  (VR). In this case, the type of questions that have to be answered are more complex and require a multi-step reasoning procedure. For example, given an image containing objects of different shapes and color, the task of recognizing the color of an object of certain shape that lies in a certain area w.r.t. the position of another object of  certain shape and color falls to the category of VR (in this case,  first  the ``source'' object must be detected, then  the ``target'' object, and, finally, its color must be recognized).
Similar to the case of VQA, a number of VR works has drawn inspiration from symbolic AI-based ideas. 


In general, many VR works are based on Neural Module Networks (NMNs) which are NNs of adaptable architecture, the topology of which is determined by the parsing of the question that has to be answered. NMNs simplify  complex questions into simpler sub-questions (sub-tasks), which can be more easily addressed. The modules that constitute the MNMs are pre-defined neural networks that implement the  functions that are required for the tackling of sub-tasks, which are assembled into a layout dynamically.  Central to many MNMs  is the utilization of prior \textit{symbolic} (structured) knowledge, which  facilitates  the handling of the sub-tasks.

Hu et al. (\citeyear{Hu2017}) propose End-to-End Module Networks as a variation of NMNs. The network first uses  coarse functional expressions describing the structure of the  computation required for the answering and, then, refines it according to the textual input in order to assemble the network. For example, for the  question \textit{``how many other objects of the same size as the purple cube exist?}'', first   crude functional expression for counting and relocating would be predicted as relevant to the answering of the question which, subsequently,  would be refined by  the parameters  from text analysis (in this case one such parameter is the color of the cube).

Similarly, Johnson et al. (\citeyear{johnson2017inferring}) propose  a variation of  NMNs, which  is  based on  the concept of~\textit{programs}. Programs are symbolic structures of certain specification written in a Domain-Specific Language and are defined by a syntax and  semantics. In the context of VR, programs  describe   a sequence of functions that must be executed, in order for an answer to be computed. During testing on the CLEVR dataset the model exhibited notable performance,  generalizing better in a variety of settings, such as for new question types and human-posed questions. Building on the notion of programs, Yi et al. (\citeyear{Yi2018}) further incorporated knowledge regarding the structural scene representation of the image. The method achieved near-perfect accuracy, while also providing transparency to the reasoning process.
 
%Another important work related to the previous is \cite{Yi2018} in which programs are extended   by  incorporating    knowledge regarding the structural scene representaton of the image. In this case, the program engine, drawing inspiration from \cite{johnson2017inferring}, is implemented as a collection of deterministic, generic functional modules in Python, which encompass all logic operations w.r.t.  questions contained in the dataset.   The  method achieved a  high  performance on the CLEVR dataset ( the method achieved 	near-perfect accuracy and outperformed the other competitive methods on every question typel) while exhibiting a better data- and memory-efficiency and providing full transparency to the reasoning process.  


An alternative NN-based approach for  VR is found in~\cite{Santoro2017}, where the incorporation of Relation Networks (RNs) in  CNNs and Long Sort-Term Memory (LSTM) architectures is proposed. RNs are architectures whose computations focus explicitly on relational reasoning and are characterized by three important features: they can infer relations, they are data efficient, and they operate on a set of objects, a  flexible symbolic input format that is agnostic to the kind of inputs it receives. For example, an object could correspond to the background, to a particular physical object, a texture, conjunctions of physical objects etc. 

To conclude, it is worth indicating also a recent trend in visual explanation approaches that couples data-driven systems with Answer Set Programming (ASP). ASP is a non-monotonic logical formalism oriented towards hard search problems. A number of studies have emerged that combine ASP abductive or inductive reasoning for the VQA domain, especially for cases when training data are not many (see e.g., \cite{SuchanMehul17,RileySridharan19,BasuShakerinGupta20})


\subsection{The Web as a Problem-Agnostic Source of Data}
As the recent renaissance in AI is partly due to the availability of big volumes of training data, along with the computational power to analyze them, it is only reasonable to expect that data-driven approaches will turn their attention to the Web in order to collect the data needed. Although the benefits mentioned in the previous sections are still achievable, the challenges faced when using a Web repository rather than a custom-made KB are now different.

The vast majority of large-scale Web repositories are not problem-specific, containing a lot of irrelevant information for a ML system to be trained correctly. For the time being, ML systems are highly specific, excelling only when trained for a particular task and tested on similar to the training conditions. As a result, state-of-the-art approaches try to rely on the semantics of structured KBs, in order to filter out noisy or irrelevant knowledge, by integrating external knowledge when visual information is not sufficiently reliable for conclusion making.

%\textit{add a group of SotA papers that take advantage of the structure and semantics of Semantic Web repositories to solve CV tasks.}
\subsubsection{Exploitation of Web-based Knowledge Graphs and Semantic Repositories}

There exists a multitude of studies that use external knowledge from structured or semi-structured Web resources, in order to answer visual queries or to perform cognitive tasks. A characteristic example is found in \cite{li2017incorporating}, where the ConceptNet KG, a semantic repository of commonsense Linked Open Data, is used to answer open domain questions on entities 
% not always visible on an image, 
such as ``\textit{What is the dog's favorite food?}''. The approach proceeds in a step-wise manner: first, visual objects and keywords are extracted from an image, using a Fast-RCNN for the objects and a LSTM for the syntactical analysis; then, queries to ConceptNet provide properties and values for the entities found in the image. When an answer is considered correct, a Dynamic Memory Network, which is an embedding vector space that contains vector representations of symbolic knowledge triples, is renewed for future encounter of the same query. In a rather similar style, Wu et al. (\citeyear{wu2016ask}) extract properties from DBpedia, by retrieving and performing semantic analysis on the comment boxes of relevant Wikipedia pages. Here, a CNN performs object detection on the image, whereas a pre-trained RNN correlates attributes to sentence descriptions. 

The approach presented in~\cite{shah2019kvqa} is the first attempt to answer a more knowledge-intensive category of questions, such as \textit{``Who is to the left of Barack Obama?}'' or `\textit{`Do all the people in the image have a common occupation?''}. These questions make reference to the named entities contained in an image, e.g., Barack Obama, White House, France etc. and require large KBs to retrieve the relevant information. In this case, the authors choose Wikidata, an RDF repository. They first extract named entities and then try to connect them with a Wikidata entity using SPARQL queries. In addition, they extract  spatial relations with other entities shown in the image and feed them to a Bi-LSTM. A multi-layered perceptron calculates the prediction for an answer, taking as input the output of the LSTM, along with the SPARQL results.% The approach achieve good results on an average score of 53.92\% over 10 different categories of questions.


\subsubsection{Aligning Data Obtained from Diverse Online Sources}

Entity resolution, also known as instance matching, concerns the task of identifying which entities across different KBs refer to the same individual. As the Web is growing in size, this problem is becoming crucial, especially in application domains that need to integrate and align knowledge obtained from various sources. An increasing number of CV studies face this problem, in an attempt to interpret visual information based on commonsense, non-visual knowledge.

Two characteristic approaches are given in \cite{chernova2017situated} and \cite{young2017making} that try to assign labels to a visual scene using Bayesian Logic Networks (BLNs) and relying on commonsense knowledge.
In \cite{chernova2017situated}, knowledge is extracted from WordNet, ConceptNet, and Wikipedia. WordNet is utilized in order to disambiguate seed words returned by the CV annotator with the aid of their hypernym. ConceptNet properties, such as $IsLocatedIn$ or $UsedFor$ that may point the location of an object, are also retrieved. With this method, the system can generate a compact semantic KB given only a small number of objects. 

In \cite{young2017making}, a CNN trained on ImageNet is used to annotate objects recognized in images. The system is capable of assigning semantic categories to specific regions, by relying on DBpedia comment boxes to calculate the semantic relatedness between objects. As expected, high accuracy of such an approach is difficult to achieve, due to the diversity of information retrieved from DBpedia; consequently, smarter ways of identifying only the relevant part of the comment boxes need to be devised.



 


==> explainability.tex <==
%%% CURRENTLY EDITED BY: 

\section{Explainability in Reasoning}

\textit{Message: Develop XAI methods that clarify the process of inferencing, a core target in AI}

\textit{Mention some VQA papers, where scene understanding is based on the semantic analysis of the surrounding objects. But also add papers that improve NNs with explainable features}
